Feature Graph Learning for 3D Point Cloud Denoising

Identifying an appropriate underlying graph kernel that reflects pairwise similarities is critical in many recent graph spectral signal restoration schemes, including image denoising, dequantization, and contrast enhancement. Existing graph learning algorithms compute the most likely entries of a properly defined graph Laplacian matrix $\mathbf{L}$, but require a large number of signal observations $\mathbf{z}$'s for a stable estimate. In this work, we assume instead the availability of a relevant feature vector $\mathbf{f}_i$ per node $i$, from which we compute an optimal feature graph via optimization of a feature metric. Specifically, we alternately optimize the diagonal and off-diagonal entries of a Mahalanobis distance matrix $\mathbf{M}$ by minimizing the graph Laplacian regularizer (GLR) $\mathbf{z}^{\top} \mathbf{L} \mathbf{z}$, where edge weight is $w_{i,j} = \exp\{-(\mathbf{f}_i - \mathbf{f}_j)^{\top} \mathbf{M} (\mathbf{f}_i - \mathbf{f}_j) \}$, given a single observation $\mathbf{z}$. We optimize diagonal entries via proximal gradient (PG), where we constrain $\mathbf{M}$ to be positive definite (PD) via linear inequalities derived from the Gershgorin circle theorem. To optimize off-diagonal entries, we design a block descent algorithm that iteratively optimizes one row and column of $\mathbf{M}$. To keep $\mathbf{M}$ PD, we constrain the Schur complement of sub-matrix $\mathbf{M}_{2,2}$ of $\mathbf{M}$ to be PD when optimizing via PG. Our algorithm mitigates full eigen-decomposition of $\mathbf{M}$, thus ensuring fast computation speed even when feature vector $\mathbf{f}_i$ has high dimension. To validate its usefulness, we apply our feature graph learning algorithm to the problem of 3D point cloud denoising, resulting in state-of-the-art performance compared to competing schemes in extensive experiments.

==> 04_algorithm.tex <==
% overview of our algorithm
% This should be the section on optimization only: given available patches and features, how to u actually denoise.
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{images/flow_chart.pdf}
    \caption{The flowchart of the proposed point cloud denoising algorithm. The input noisy point cloud will go through (2)(3)(4)(5) in each iteration. }
    \vspace{-0.1in}
    \label{fig:flowchart}
\end{figure*}

Having formulated the problem for point cloud denoising, we propose to solve (\ref{eq:formulation_final}) by alternately optimizing the point cloud $\mathbf{Y}$ and the underlying graph $\mathbf{L}$. 
The iterations terminate when the difference in the objective between two consecutive iterations stops decreasing. 
Parameter settings are presented in Section~\ref{sec:results}.
% As shown in Fig.~\ref{fig:flowchart}, the input goes through four steps in order: 
% 1) \textit{normal estimation}, to estimate point normals \cite{hoppe92} as one feature for each 3D point; 
% 2) \textit{patch construction}, to segment the entire point cloud into 3D patches via $k$-NN search; 
% 3) \textit{feature graph learning}, to build graph connectivities over each 3D patch and then learn edge weights; 
% 4) \texit{point cloud optimization}, to solve the formulated optimization problem with the graph learnt from step 3, which leads to the denoised point cloud. 
% \red{u need to select the patches first before u have the optimization in (38). u also have connectivity decided, based on selected patches, and the ``feature metric learning" just decide on edge weights based on chosen connectivity.
% Move your patch construction and your graph construction subsections up to section 5.}

\subsection{Optimizing the point cloud $\mathbf{Y}$}
In the first iteration, we initialize the graph Laplacian matrix $\mathbf{L}$ from the input $\mathbf{P}$ by constructing a $k$-nearest-neighbor ($k$NN) graph, and thus fix $\mathbf{L}$ in (\ref{eq:formulation_final}). 
Next, taking the derivative of (\ref{eq:formulation_final}) with respect to the three components of $\vec{Y}$, $\{\vec{Y}_x,\vec{Y}_y,\vec{Y}_z\}$, we have
\begin{equation}
\begin{array}{c}
    (\gamma \mathcal{T}^{\top}\mathbf{L}\mathcal{T} + \mathbf{I})\vec{Y}_x=\vec{P}_x+\gamma \mathcal{T}^{\top} \mathbf{L} \mathbf{C}_x, \\
    (\gamma \mathcal{T}^{\top}\mathbf{L}\mathcal{T} + \mathbf{I})\vec{Y}_y=\vec{P}_y+\gamma \mathcal{T}^{\top} \mathbf{L} \mathbf{C}_y, \\
    (\gamma \mathcal{T}^{\top}\mathbf{L}\mathcal{T} + \mathbf{I})\vec{Y}_z=\vec{P}_z+\gamma \mathcal{T}^{\top} \mathbf{L} \mathbf{C}_z,
\end{array}
\label{eq:sol}
\end{equation}
where $\mathbf{I}$ is an identity matrix. 
(\ref{eq:sol}) can be treated as three linear equation sets and thus can be efficiently solved using conjugate gradient (CG) methods, such as the LSQR algorithm \cite{paige1982lsqr}. 
The acquired solution of $\vec{Y}$ is then used to update $\mathbf{L}$ in the subsequent iteration. 

\subsection{Optimizing the graph $\mathbf{L}$}

When $\vec{Y}$ is fixed, the learning of $\mathbf{L}$ follows the optimization:
\begin{equation}
\min_{\mathbf{L}}
    \text{tr}((\mathcal{T} \vec{Y} - \mathbf{C})^{\top}\mathbf{L} (\mathcal{T} \vec{Y} - \mathbf{C})),
    \label{eq:optimize_L}
\end{equation}
which is the formulation of feature graph learning. 

An algorithmic summary of the proposed feature graph learning for point cloud denoising is presented in Algorithm~\ref{alg:denoising}.

\begin{algorithm}[htb]
  \caption{Block Gradient Descent}
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \label{alg:block_descent}
    \Input{Feature matrix $\vec{f} \in \mathbb{R}^{N\times K}$, graph signals $\mathbf{z} \in \mathbb{R}^N$, constraint $C$} 
    \Output{Positive definite matrix $\mathbf{M} \in \mathbb{R}^{K \times K}$}
    Initialize $\mathbf{M}$ with a diagonal matrix whose elements are $C/K$ \\
    \For{$i=1$ to $K$}{
      Swap the $1^\text{st}$ row and the $i^\text{th}$ row of $\mathbf{M}$; \\
        Initialize $\mathbf{U}_t$ with $\hat{\mathbf{U}}_t$ \\
        Select $M$ points (set $\mathbf{C}_t$) as patch centers; \\
        \For{$\mathbf{c}_l$ in $\mathbf{C}_t$}{
            Find $k$-nearest neighbors of $\mathbf{c}_l$; \\
            Build patch $\hat{\mathbf{p}}_{t,l}$; \\
            Add $\hat{\mathbf{p}}_{t,l}$ to $\hat{\mathbf{P}}_t$; \\
        }
            \Repeat{convergence}{
            \For{$\hat{\mathbf{p}}_{t,l}$ in $\hat{\mathbf{P}}_t$}{
                \For {$\hat{\mathbf{p}}_{t, j}$ in $\hat{\mathbf{p}}_{t,l}$'s adjacent patches}{
                    Calculate the similarity metric $s_{l, j}$ between $\hat{\mathbf{p}}_{t,l}$ and $\hat{\mathbf{p}}_{t, j}$ as in Eq.~(\ref{eq:similarity}); \\
                    Connect nearest points in $\hat{\mathbf{p}}_{t,l}$ and $\hat{\mathbf{p}}_{t, j}$ with the edge weight $s_{l, j}$; \\
                }
                Search the corresponding patch $\hat{\mathbf{p}}_{t-1,l}$ of $\hat{\mathbf{p}}_{t,l}$ in the previous frame, which is the most similar to $\hat{\mathbf{p}}_{t,l}$ in terms of the metric metric $s_{(t-1)l, tl}$ as in Eq.~(\ref{eq:similarity}); \\
                Connect corresponding points in $\hat{\mathbf{p}}_{t,l}$ and $\hat{\mathbf{p}}_{t-1, l}$ with the edge weight $s_{(t-1)l, tl}$; \\
            }
            Compute the intra-frame graph Laplacian $\mathbf{L}_t$; \\
            Compute the weight matrix $\mathbf{W}_{t,t-1}$ between corresponding patches; \\
            Solve Eq.~(\ref{eq:closed_form_U}) to update $\mathbf{U}_t$; \\
        }
    }
\end{algorithm}

% where $\mathbf{c}=[c_1,...,c_m]^T$, and $\mathbf{c}^T\mathbf{M}\mathbf{c}$ is its
% Mahalanobis distance with a matrix $M$. The domain of $M$ is the cone of positive
% semi-definite matrices. Both the objective and constraint in (\ref{eq:optimize_c_constraint}) are convex, and thus can be solved optimally and efficiently.  

% We deploy proximal gradient descent to solve (\ref{eq:optimize_c_constraint}). Firstly, we compute the gradient of the objective $g(\mathbf{M})$:
% \begin{equation}
%     \bigtriangledown g(\mathbf{M}) = -\sum_{\{i,j\}} \exp\{-(\mathbf{f}_i-\mathbf{f}_j)^T \mathbf{M} (\mathbf{f}_i-\mathbf{f}_j) \}d_{i,j} \cdot (\mathbf{f}_i-\mathbf{f}_j)(\mathbf{f}_i-\mathbf{f}_j)^T
% \end{equation}

% According to the constraint in (\ref{eq:optimize_c_constraint}), we project onto the convex spectral set:
% \begin{equation}
%     T = \{\mathbf{M} \succeq 0 ~|~ \text{tr}(\mathbf{M}) \leq C\}
% \end{equation}
% The proximal projection onto $T$ is given by
% \begin{equation}
% \begin{split}
% \Pi_T(\mathbf{M}) &=\mathbf{U} \textbf{diag}(\Pi_S(\sigma(\mathbf{M}))) \mathbf{U}^T \\ &=\sum_{i=1}^K \text{min}\{\text{max}\{\lambda_i,0\},C\}\mathbf{u}_i\mathbf{u}_i^T,
% \end{split}
% \end{equation}
% where $\mathbf{U}$ is the matrix of eigenvectors $\mathbf{u}_i$ of $\mathbf{M}$ and $\sigma(\mathbf{M})$ is the diagonal matrix of eigenvalues $\lambda_i$ of $\mathbf{M}$. The operation of $\text{max}\{\lambda_i,0\}$ ensures $\mathbf{M}$ is positive semi-definite, while $\text{min}\{\cdot,C\}$ is necessary for the constraint $\text{tr}(\mathbf{M}) \leq C$.

% We then have the PG iteration:
% \begin{equation}
%     \mathbf{M}^{l+1} := \Pi_T(\mathbf{M}^l - t \bigtriangledown g(\mathbf{M}^l)).
% \end{equation}

   
% \begin{equation}
% \begin{split}
% &\min_{c_1,c_2}
%     \sum_{\{i,j\}}\exp{\left(-c_1\|\vec{p}_s-\vec{p}_t\|_2^2-c_2\left| \sin \left \langle \mathbf{n}_s, \mathbf{n}_t \right \rangle \right| \right)}\|\mathbf{p}_i-\mathbf{p}_j\|_2^2+\beta\|\mathbf{c}\|_2^2,\\
% & \quad \text{s.t.} \quad \, c_1 \geq 0, c_2 \geq 0.
% \label{eq:optimize_c_constraint}
% \end{split}
% \end{equation}
 

%a function of the angle between the normals of neighboring points into the weight function.  



%In (\ref{eq:graph_weight}), the exponential term describes the relative distance between $\mathbf{p}_i$ and $\mathbf{p}_j$, as widely adopted in the literature. Further, the cosine term captures the similarity between the direction of normals at $\mathbf{p}_i$ and $\mathbf{p}_j$. If the normal angle is large and even reaches $\pi/2$, then the cosine term tends to $0$, resulting in a small weight even when the relative distance between $\mathbf{p}_i$ and $\mathbf{p}_j$ is small. Hence, this term penalizes corresponding points with large difference in the normal direction, i.e., when the two points reside on local surfaces with different orientations. We apply the PCA-based method \cite{hoppe92} to estimate surface normals from point clouds based on local neighborhoods of each point, which is robust to noise.  
%
%In particular, $\sigma$ decides the radius of the neighborhood and the distribution of edge weights, which has substantial impact on the denoising performance. 

%\begin{equation}
%\min_{\sigma}
%    \sum_{\{i,j\}}\sum_{c \in \{x,y,z\}}\exp{\left(-\frac{\|\mathbf{p}_i-\mathbf{p}_j\|^2}{ \sigma ^2}\right)} \cdot \left| \cos \left \langle \mathbf{n}_s, \mathbf{n}_t \right \rangle \right|(p_s^c-p_t^c)^2.
%    \label{eq:optimize_L}
%\end{equation}






% \subsection{Computational Complexity Analysis}

% The computational complexity of our algorithm can be deduced as follows:
% \begin{itemize}
%     \item We use KD-tree for the $k$-nearest-neighbor searches. The cost of the $k$-nearest-neighbor search for all points is $\mathcal{O}(kN \log N)$.
%     \item We need to run the RPCA solver to estimate the normal on each point using its $k$-nearest-neighbor. The cost of the RPCA solver on each point is $\mathcal{O}(tk)$ \cite{mattei}, where $t$ is the number of iterations. For all points, the cost is $\mathcal{O}(tkN)$.
%     \item Constructing $M$ patches still requires $k$-NN search, and the cost is $\mathcal{O}(kM \log N)$.
%     \item For graph construction, the $\varepsilon$-nearest-patch to be connected can be found in $\mathcal{O}(\varepsilon M \log M)$ time.
%     \item For the weight computation, the cost is $\mathcal{O}(\varepsilon k^2 M)$.
%     \item The cost of CG-based algorithm to solve the optimization problem is $\mathcal{O}(m \sqrt{\kappa})$ \cite{shewchuk1994introduction}, where $m$ is the number of non-zero entries in the matrix, and $\kappa$ is the condition number of the matrix. In our problem, the Laplacian matrix is sparse, and thus $m \ll N^2$.
% \end{itemize}

% Overall, the running time of our algorithm depends on four parameters (1) the number of nearest neighbors, (2) the number of iterations to run the RPCA normal estimation, (3) the number of patches, and (4) the number of nearest patch neighbors.

% \subsection{Spectral Domain Analysis}

% We shed light on the solution in (\ref{eq:sol}) in the spectral domain. Since $\mathcal{T} \in \{0,1\}^{(k+1)M \times N}$ is a selection matrix, $\mathcal{T}^{\top} \mathbf{L} \mathcal{T}$ can be treated as a principle submatrix of $\mathbf{L}$, denoted by $\mathbf{L}^{'}$. Hence, the sub-Laplacian matrix $\mathbf{L}^{'}$ is also a real symmetric matrix, which admits a set of real eigenvalues $ \{\lambda_l\}_{l=0,1,...,n-1}, \lambda_0=0 \leq \lambda_1 \leq ... \lambda_{n-1}$, with a complete set of orthonormal eigenvectors $\{\mathbf{\psi}_l\}_{l=0,1,...,n-1} $, \textit{i.e.}, $\mathbf{L}^{'}\mathbf{\psi}_l=\lambda_l\mathbf{\psi}_l $, for $l=0,1,...,n-1$. Note that the eigenvalues $ \{\lambda_l\}$ are known as the spectrum of the graph. Then the filtering kernel in (\ref{eq:sol}) can be written in the spectral domain as  

% \begin{equation}
% \hat{\lambda_l} = \frac{1}{1 + \gamma \lambda_l}.
% \end{equation}

% As $ \lambda_0=0 $, $ \hat{\lambda_0}=1 $. As $ \lambda_l $ increases, $ \hat{\lambda_l} $ decreases, which corresponds to stronger filtering strength. 
% Since larger $ \lambda_l $ corresponds to higher frequency, stronger filtering is performed on higher-frequency components, thus attenuating noise more as noise generally lies in the sub-band of higher frequencies. 

% % \subsection{Normal Estimation}
% % In our proposed algorithm, normals are mainly used to measure the similarity of adjacency patches, because normals enable efficient representation of the structure of the underlying surface. However, it is challenging to compute noise-free normals given a noisy point cloud. A popular PCA-based method \cite{hoppe92} estimates surface normals from point clouds  based on local neighborhoods of each point. We apply this method to calculate normals for each point on the entire point cloud, denoted by $\mathcal{N}=\{\mathbf{n}_1, \mathbf{n}_2, ..., \mathbf{n}_N\}$ with $\mathbf{n}_i$ meaning the normal of the $i$-th point. $\mathbf{P}=\{\mathbf{p}_1, \mathbf{p}_2, ..., \mathbf{p}_n\}$ with $\mathbf{p}_i \in \mathbb{R}^3$ meaning the coordinates of the $i$-th point.


==> backup_block.tex <==
\subsection{Problem Formulation}

Conceptually, an edge weight $w_{i,j}$ reflects the similarity between samples at nodes $i$ and $j$; specifically, using the commonly used Gaussian kernel \cite{shuman13spm}, edge weight $w_{i,j} = \exp \left\{ - \delta_{i,j} \right\}$, where $\delta_{i,j}$ denotes the estimated feature distance between samples $i$ and $j$.
One advantage of the Gaussian kernel is that edge weight $w_{i,j}$ is in range $[0,1]$, ensuring the resulting combinatorial graph Laplacian matrix $\mathbf{L}$ to be \textit{positive semi-definite} (PSD) \cite{cheung2018graph}.

The feature distance between samples essentially measures the inter-sample similarity.    
As one well-known example of feature distance, consider the \textit{bilateral filter} in image denoising \cite{tomasi1998bilateral} %\red{cite Tomasi's paper} \blue{added.} 
that employs pixel intensities $x_i$ and pixel locations $\mathbf{l}_i$ as relevant features to compute $\delta_{i,j}$, namely,
\begin{align}
\delta_{i,j} = \frac{(x_i - x_j)^2}{\sigma_x^2} + \frac{\|\mathbf{l}_i - \mathbf{l}_j\|_2^2}{\sigma_l^2},
\label{eq:bf}
\end{align}
where $\sigma_x$ and $\sigma_l$ are parameters. 
Defining $\mathbf{f}_i = [x_i ~~ \mathbf{l}_i]^{\top}$, we can rewrite \eqref{eq:bf} in matrix form as:
\begin{align}
\delta_{i,j} = \left( \mathbf{f}_i - \mathbf{f}_j \right)^{\top} 
\left[ \begin{array}{cc}
1/\sigma_x^2 & 0 \\
0 & 1/\sigma_l^2
\end{array}
\right]
\left( \mathbf{f}_i - \mathbf{f}_j \right).
\end{align}
\cite{tomasi1998bilateral} shows that with appropriate parameters $\sigma_x$ and $\sigma_l$, the bilateral filter can achieve very good edge-preserving image denoising performance. 
How to best determine $\sigma_x$ and $\sigma_l$, however, was left unanswered.

%However, in cases where certain features contribute more to the specific task (e.g., the feature of coordinates is more crucial than the feature of colors for point cloud denoising), the measurement in the Euclidean distance does not distinguish different features. 
More generally, associated with each sample $i$ is a length-$K$ vector of relevant features, and our goal is to compute an optimal \textit{Mahalanobis distance} for the given features: 
\begin{equation}
    \delta_{i,j} = (\mathbf{f}_i-\mathbf{f}_j)^{\top} \mathbf{M} (\mathbf{f}_i-\mathbf{f}_j),
    \label{eq:graph_weight}
\end{equation}
where $\mathbf{M} \in \mathbb{R}^{K \times K}$ is a \textit{positive definite} (PD) matrix\footnote{PD is desirable, so that if $\mathbf{f}_i - \mathbf{f}_j \neq \mathbf{0}$, then $(\mathbf{f}_i-\mathbf{f}_j)^{\top} \mathbf{M} (\mathbf{f}_i-\mathbf{f}_j) > 0$.}. 
%
%as applying a linear transformation of the input data \cite{kulis2013metric}: since $\mathbf{M}$ is PSD, it can be factorized as $\mathbf{M}=\mathbf{G}^{\top}\mathbf{G}$, which converts the distance to $\| \mathbf{G} \mathbf{f}_i -\mathbf{G} \mathbf{f}_j \|_2^2$. Thus the Mahalanobis distance is able to capture the distance of intrinsic features via the linear transformation.   
%
As a special case, when $\mathbf{M}$ is a diagonal matrix with positive diagonal entries, the definition in (\ref{eq:graph_weight}) defaults to that in \cite{yang2018apsipa}. 
Diagonal $\mathbf{M}$ can capture the relative importance of individual features when computing $\delta_{i,j}$, but fails to capture possible cross-correlation among features, and thus is sub-optimal in the general case.     

We can now pose an optimization problem for $\mathbf{M}$ according to (\ref{eq:rgssp}): 
we seek the optimal metric $\mathbf{M}$ that yields the smallest GLR term given feature vector $\mathbf{f}_i$ for each node $i$, and one (or more) signal observation(s) $\mathbf{z}$.
Specifically, denote by $d_{i,j} = (z_i-z_j)^2$ the inter-node sample difference square of observation $\mathbf{z}$, we have 
\begin{equation}
\begin{split}
&\min_{\mathbf{M}}
    \sum_{\{i,j\}}\exp\{-(\mathbf{f}_i-\mathbf{f}_j)^{\top} \mathbf{M} (\mathbf{f}_i-\mathbf{f}_j) \}d_{i,j}\\
& \text{s.t.} \quad \, \mathbf{M} \succ 0.
\label{eq:optimize_L_new}
\end{split}
\end{equation}
If there are more than one signal observations $\mathbf{z}^1, \ldots, \mathbf{z}^S$ available, then $d_{i,j}$ in \eqref{eq:optimize_L_new} can be easily generalized to be the sum of inter-node sample difference square of all observations, i.e. $d_{i,j} = \sum_{s=1}^S (z_i^s-z_j^s)^2$.

Minimizing (\ref{eq:optimize_L_new}) directly would lead to one pathological solution, i.e., $m_{i,i}=\infty, \forall i$, resulting in edge weights $w_{i,j} = 0$. 
Topologically, this means nodes in the graph are all isolated, resulting in no inter-sample correlation across nodes. 
%\red{filtering does not make sense in this context. need to fix this.} \blue{fixed.}
To avoid this solution, we enforce the trace of $\mathbf{M}$ to be smaller than a constant parameter $C$, resulting in
\begin{equation}
\begin{split}
&\min_{\mathbf{M}}
    \sum_{\{i,j\}}\exp\{-(\mathbf{f}_i-\mathbf{f}_j)^{\top} \mathbf{M} (\mathbf{f}_i-\mathbf{f}_j) \}d_{i,j}\\
& \text{s.t.} \quad \,\mathbf{M} \succ 0; \;\;\;
\text{tr}(\mathbf{M}) \leq C.
\label{eq:optimize_c_constraint}
\end{split}
\end{equation}

\subsection{Block Coordinate Iteration}

%\red{this subsection B is way too long. u need to split into more subsections. after ``problem formulation", try ``Block Coordinate Iteration", then ``Gershgorin-based Reformulation", then ``Algorithm Development". } 
To solve \eqref{eq:optimize_c_constraint}, we design a block gradient descent algorithm. 
First, we divide $\mathbf{M}$ into four sub-matrices:
\begin{equation}
\mathbf{M} = \begin{bmatrix}
m_{1,1} & \mathbf{M}_{1,2} \\
\mathbf{M}_{2,1} & \mathbf{M}_{2,2} 
\end{bmatrix},
\label{eq:submatrix}
\end{equation}
where $m_{1,1} \in \mathbb{R}$, $\mathbf{M}_{1,2} \in \mathbb{R}^{1 \times (K-1)}$, $\mathbf{M}_{2,1} \in \mathbb{R}^{(K-1) \times 1}$ and $\mathbf{M}_{2,2} \in \mathbb{R}^{(K-1) \times (K-1)}$. 
%\red{feature is a length-$K$ vector. this is because the signal is length-$N$, so to avoid confusing, we should use $K$ instead of $n$.} \blue{fixed.}
We assume $\mathbf{M}$ is symmetric, i.e., $\mathbf{M}_{1,2} = \mathbf{M}_{2,1}^{\top}$.     
Our strategy is to optimize one row and column represented by $m_{1,1}$ and $\mathbf{M}_{2,1}$ in one iteration, given objective and constraints in \eqref{eq:optimize_c_constraint}. 
In the next iteration, a different row and column is selected, and with appropriate rows and columns reordering, the optimization variables $m_{1,1}$ and $\mathbf{M}_{2,1}$ can still reside in the first row and column as shown in \eqref{eq:submatrix}.
%\red{r u using notation $\mathbf{M}_{1,2}$ or $\mathbf{M}_{1,2}$? u were using $w_{i,j}$, not $w_{ij}$, earlier. should be consistent.}

By the \textit{Haynsworth inertia additivity} \cite{haynsworth1968determination}, a symmetric real matrix $\mathbf{M}$ is PD if and only if both its sub-matrix $\mathbf{M}_{2,2}$ and its corresponding Schur complement $m_{1,1} - \mathbf{M}_{2,1}^{\top} \mathbf{M}_{2,2}^{-1} \mathbf{M}_{2,1}$ are PD. 
Hence, we can ensure $\mathbf{M}$ is PD by constraining the Schur complement  $m_{1,1} - \mathbf{M}_{2,1}^{\top} \mathbf{M}_{2,2}^{-1} \mathbf{M}_{2,1}$ to be positive, given that sub-matrix $\mathbf{M}_{2,2}$ is PD from the previous iteration.

In the first iteration, we initialize $\mathbf{M}$ to be a diagonal matrix with each diagonal entry $m_{i,i}=C/K$, thus ensuring $\mathbf{M}$ is PD and $\mathrm{tr}(\mathbf{M}) \leq C$.
%\red{don't do random! this is the most obvious initialization!}
In each subsequent iteration, we impose a positivity constraint on the Schur complement of a submatrix $\mathbf{M}_{2,2}$ as follows:
\begin{equation}
    m_{1,1} - \mathbf{M}_{2,1}^{\top} \mathbf{M}_{2,2}^{-1} \mathbf{M}_{2,1} > 0.  
\end{equation}
Optimization problem \eqref{eq:optimize_c_constraint} thus becomes:   
\begin{equation}
\begin{split}
&\min_{m_{1,1},\mathbf{M}_{2,1}}
    \sum_{\{i,j\}}\exp\left\{-({\mathbf{f}}_i-{\mathbf{f}}_j)^{\top} \mathbf{M}({\mathbf{f}}_i-{\mathbf{f}}_j) \right\}d_{i,j}\\
& \text{s.t.} \quad \,m_{1,1}-\mathbf{M}_{2,1}^{\top} \mathbf{M}_{2,2}^{-1} \mathbf{M}_{2,1} > 0, \\ 
& ~~~~~~~m_{1,1} \leq C - \text{tr}(\mathbf{M}_{2,2}).
\end{split}  
\label{eq:schur}
\end{equation}

Given $\mathbf{M}_{2,2}$ is fixed in \eqref{eq:schur},  we can simplify the objective as follows. 
Let $\mathbf{g}_{ij} = \mathbf{f}_i-{\mathbf{f}}_j$, $\mathbf{g}_{ij} \in \mathbb{R}^K$.
Writing $\mathbf{M}$ in terms of its four sub-matrices in \eqref{eq:submatrix}, we simplify the objective via matrix multiplication as 
\begin{equation}
    \sum_{\{i,j\}} 
\exp\{- (\mathbf{g}_{ij}(1)^2 m_{1,1} + 2 \mathbf{g}_{ij}(1) \mathbf{M}_{2,1}^{\top} \mathbf{g}_{ij}(2))\}\tilde{d}_{i,j}
\end{equation}
% \begin{align}
% \sum_{\{i,j\}} 
% \exp\{&- (\mathbf{g}_{ij}(1)^2 m_{1,1} + 2 \mathbf{g}_{ij}(1) \mathbf{M}_{2,1}^{\top} \mathbf{g}_{ij}(2) \nonumber \\
% & +\mathbf{g}_{ij}(2)^{\top} \mathbf{M}_{2,2} \mathbf{g}_{ij}(2)) \}d_{i,j},
% \end{align}
where $\tilde{d}_{i,j}=\exp\{-\mathbf{g}_{ij}(2)^{\top} \mathbf{M}_{2,2} \mathbf{g}_{ij}(2) \}d_{i,j}$ is a constant as $\mathbf{M}_{2,2}$ is fixed in the iteration.
%\red{I thought u r going to lump the exponential term involving the constant $\mathbf{M}_{2,2}$ into $d_{i,j}$ and call it a new term like $\tilde{d}_{i,j}$. } \blue{edited.}
$\mathbf{g}_{ij}(1)$ denotes the first entry in vector $\mathbf{g}_{ij}$, and $\mathbf{g}_{ij}(2)$ denotes the remaining entries.

\magenta{

Optimization problem \eqref{eq:optimize_c_constraint} can be rewritten as: 
\begin{equation}
    \begin{split}
&\min_{\mathbf{M}}
    \sum_{\{i,j\}}\exp\left\{-({\mathbf{f}}_i-{\mathbf{f}}_j)^{\top} \mathbf{M}({\mathbf{f}}_i-{\mathbf{f}}_j) \right\}d_{i,j}\\
& \text{s.t.} \quad \,m_{i,i}-\sum_{j \neq i} |m_{i,j}| > 0, \forall i, \\ 
& ~~~~~~~\text{tr}(\mathbf{M}) \leq C.
\end{split}  
\end{equation}

Let $\mathbf{g}_{ij} = \mathbf{f}_i-{\mathbf{f}}_j$, $\mathbf{g}_{ij} \in \mathbb{R}^K$.
Writing $\mathbf{M}$ in terms of its four sub-matrices in \eqref{eq:submatrix}, we simplify the objective via matrix multiplication as 
\begin{equation}
    \sum_{\{i,j\}} 
\exp\left\{-\sum_{k=1}^{K} \left( \mathbf{g}_{ij}^{2}(k)m_{k,k} + \mathbf{g}_{ij}(k)\mathbf{g}_{ij}^{\top}(\setminus k)\mathbf{M}_{\setminus k,k} \right) \right\} d_{i,j}
\end{equation}
where $\mathbf{g}_{ij}(k)$ denotes the $k$-th entry of vector $\mathbf{g}_{ij}$, $\mathbf{g}_{ij}(\setminus k)$ indicates the remaining entries of vector $\mathbf{g}_{ij}$, and $\mathbf{M}_{\setminus i, j}$ is the vector of the $j$-th column after removing $m_{i,j}$.

The above formulation can be simplified as
\begin{equation}
    \sum_{\{i,j\}} 
\exp\left\{-\sum_{k=1}^{K} \left( \mathbf{g}_{ij}^{2}(k)m_{k,k} \right) \right\} \tilde{d}_{i,j},
\end{equation}
where $\tilde{d}_{i,j}=\exp\left\{-\sum_{k=1}^{K}\mathbf{g}_{ij}(k)\mathbf{g}_{ij}^{\top}(\setminus k)\mathbf{M}_{\setminus k,k}\right\}d_{i,j}$.

Let $\mathbf{m}=[m_{1,1},...,m_{K,K}]^{\top}$, we compute the gradient of the above formulation with respect to $\mathbf{m}$:
\begin{equation}
    \bigtriangledown F(\mathbf{m})=\left[
\begin{array}{c}
   -\sum_{\{i,j\}} \exp\left\{-\sum_{k=1}^{K} \mathbf{g}_{ij}^{2}(k)m_{k,k} \right\} \mathbf{g}_{ij}^{2}(1) \tilde{d}_{i,j} \\
   \vdots \\
   -\sum_{\{i,j\}} \exp\left\{-\sum_{k=1}^{K} \mathbf{g}_{ij}^{2}(k)m_{k,k} \right\} \mathbf{g}_{ij}^{2}(K) \tilde{d}_{i,j}
  \end{array}
  \right]
\end{equation}

The constraints for $\mathbf{m}$ forms a convex set:
\begin{equation}
    \mathcal{S}=\left\{ \mathbf{m} ~\bigg|~ m_{i,i}-\sum_{j \neq i} |m_{i,j}| > 0, \sum_{i=1}^K m_{i,i}< C, \forall i \right\}.
\end{equation}

Then, we define the indicator function $I_{\mathcal{S}}(\mathbf{m})$:
\begin{equation}
   I_{\mathcal{S}}(\mathbf{m})=
    \left\{
        \begin{array}{lr} 
            0, & \mathbf{m} \in \mathcal{S}  \\
            \infty, & \text{otherwise}
        \end{array}
    \right.
\end{equation}

The proximal mapping $\Pi_{I_{\mathcal{S}}}(\mathbf{m})$ for the indicator function is a projection onto the convex set $\mathcal{S}$, i.e.,
\begin{equation}
    \Pi_{I_{\mathcal{S}}}(\mathbf{m})=
    \left\{
        \begin{array}{lr} 
            P_{\mathcal{T}}(\mathbf{m}), & \vec{1}^{\top} P_{\mathcal{T}}(\mathbf{m}) < C,  \\
            P_{\mathcal{T}}(\mathbf{m}-\alpha\cdot\vec{1}), & \text{otherwise,}
        \end{array}
    \right.
\end{equation}
where $P_{\mathcal{T}}(\mathbf{m})=\min\left\{ \max\{ m_{i,i}, \sum_{j \neq i}|m_{i,j}| \}, C \right\} \big|_{i=1}^{K}$, and $\alpha$ is any positive root of $\vec{1}^{\top}P_{\mathcal{T}}(\mathbf{m}-\alpha\cdot\vec{1}) = C$ \cite{beck2017first}.

The PG problem can be rewritten as:
\begin{equation}
    \mathbf{m}^{l+1}=\Pi_{I_{\mathcal{S}}}(\mathbf{m}^{l}-t\bigtriangledown F(\mathbf{m}^{l})).
\end{equation}

}

\subsection{LOBPCG-based Reformulation}
\red{are you using LOBPCG to compute one eigen-pair now? if so, u need to change this.}
\blue{Changed.}
Computation of a large matrix inverse $\mathbf{M}_{2,2}^{-1}$ in \eqref{eq:schur} per iteration is costly.
To avoid computing $\mathbf{M}_{2,2}^{-1}$, we derive a bound on the eigenvalues of $\mathbf{M}_{2,2}^{-1}$ to ensure the positivity constraint on the Schur complement $m_{1,1} - \mathbf{M}_{2,1}^{\top} \mathbf{M}_{2,2}^{-1} \mathbf{M}_{2,1}$ in \eqref{eq:schur} is satisfied. 

%\red{I think it is more natural to describe the eigen-decomposition of $\mathbf{M}_{2,2}$ instead of $\mathbf{M}_{2,2}^{-1}$.} \blue{I think starting from the eigen-decomposition of $\mathbf{M}_{2,2}^{-1}$ is easier to understand. }
First, since $\mathbf{M}_{2,2}^{-1}$ is a real and  symmetric PD matrix, it admits diagonalization with eigen-matrix $\mathbf{U}$ (eigenvectors as columns) and diagonal matrix $\boldsymbol{\Lambda}$ with real eigenvalues $0 < \lambda_{1} \leq \ldots \leq \lambda_{K}$ along its diagonal. 
Hence,
\begin{equation}
    \begin{split}
    \mathbf{M}_{2,1}^{\top} \mathbf{M}_{2,2}^{-1} \mathbf{M}_{2,1} 
    & = \mathbf{M}_{2,1}^{\top} \mathbf{U} \boldsymbol{\Lambda} \mathbf{U}^{\top} \mathbf{M}_{2,1} \\
    & = (\mathbf{U}^{\top} \mathbf{M}_{2,1})^{\top} \boldsymbol{\Lambda} (\mathbf{U}^{\top} \mathbf{M}_{2,1}),
    \end{split}
\end{equation}
which is essentially scaling the $l_2$-norm of $\mathbf{U}^{\top} \mathbf{M}_{2,1}$ by eigenvalues in $\boldsymbol{\Lambda}$. 
Hence, a sufficient condition to the first constraint in (\ref{eq:schur}) is to bound with the maximum eigenvalue $\lambda_{\text{max}}$ of $\mathbf{M}_{2,2}^{-1}$: 
\begin{equation}
\begin{split}
    & m_{1,1} > \lambda_{\text{max}} (\mathbf{U}^{\top} \mathbf{M}_{2,1})^{\top} (\mathbf{U}^{\top} \mathbf{M}_{2,1}) \\
    & \Rightarrow m_{1,1} > \lambda_{\text{max}} \mathbf{M}_{2,1}^{\top} \mathbf{U} \mathbf{U}^{\top} \mathbf{M}_{2,1} \\
    & \Rightarrow m_{1,1} > \lambda_{\text{max}} \mathbf{M}_{2,1}^{\top} \mathbf{M}_{2,1},
\end{split}
\end{equation}
%\red{this looks correct, though a reviewer can argue that this upper bound based on $\lambda_{\max}$ can be quite loose in the general case.} \blue{We may argue this is a sufficient condition which leads to reasonable results? }
%\red{finish your discussion on how to bound the eigenvalues and the alternative constraint first, then start a new subsection on algorithm development.}
%\red{when $\mathbf{M}_{1,2}$ is fixed, (35) becomes a linear constraint for $m_{1,1}$. when $m_{1,1}$ is fixed, the constraint becomes:
%\begin{align}
%\frac{m_{1,1}}{\lambda_{\max}} > \| \mathbf{M}_{1,2} \|_2^2
%\end{align}
%This is a convex set, in particular, a $(n-1)$ dimensional norm ball with radius $\sqrt{m_{1,1}/\lambda_{\max}}$. So u can use proximal gradient to solve for $\mathbf{M}_{1,2}$.
%}

$\lambda_{\text{max}}$ is the reciprocal of the minimum eigenvalue $\theta_{\text{min}}$ of $\mathbf{M}_{2,2}$, i.e., $\lambda_{\text{max}}=\frac{1}{\theta_{\text{min}}}$. 
We employ Locally Optimal Block Preconditioned Conjugate Gradient (LOBPCG) \cite{Knyazev01} to calculate $\theta_{\text{min}}$, which is efficient to compute the extreme eigen-pairs of a large sparse matrix with linear convergence.


% Thus, a \textit{lower bound} $\theta_{\min}^l$ for $\theta_{\min}$ will in turn lead to an \textit{upper bound} $\lambda^u_{\max} = \frac{1}{\theta^l_{\min}}$ for $\lambda_{\max}$. 
% We compute a lower bound  $\theta^l_{\text{min}}$ using the \textit{Gershgorin circle theorem} \cite{gervsgorin1931uber}. 
% In a nutshell, Gershgorin circle theorem states that each eigenvalue of a matrix $\mathbf{H} = \mathbf{M}_{2,2}$ must reside in one Gershgorin disc with centre $c_i$ and radius $r_i$ corresponding to a row $i$ in $\mathbf{H}$, where $c_i$ and $r_i$ are computed as:
% \begin{align}
% c_i = h_{i,i},  ~~~~
% r_i = \sum_{j~|~j\neq i} |h_{i,j}|
% \end{align}

% This means that $\theta_{\text{min}}$ must be lower-bounded by the smallest left-end of all Gershgorin discs, i.e., 
% \begin{equation}
%     \theta_{\text{min}} \geq \min_i (c_i - r_i) 
%     = \theta^l_{\min}
% \label{eq:theta}
% \end{equation}
Having computed $\theta_{\min}$ from $\mathbf{M}_{2,2}$ without eigen-decomposition, we can reformulate (\ref{eq:schur}) as    
\begin{equation}
\begin{split}
&\min_{m_{1,1},\mathbf{M}_{2,1}}
    \sum_{\{i,j\}} 
\exp\{- (\mathbf{g}_{ij}(1)^2 m_{1,1} + 2 \mathbf{g}_{ij}(1) \mathbf{M}_{2,1}^{\top} \mathbf{g}_{ij}(2))\}\tilde{d}_{i,j}\\
& \text{s.t.} \quad \,m_{1,1} > \frac{1}{\theta_{\min}} \mathbf{M}_{2,1}^{\top} \mathbf{M}_{2,1}, \\ 
& ~~~~~~~m_{1,1} \leq C - \text{tr}(\mathbf{M}_{2,2}).
\end{split}  
\label{eq:constrained_final}
\end{equation}
Next, we design an efficient algorithm to address (\ref{eq:constrained_final}). 


\subsection{Algorithm Development}

In each iteration of the block descent algorithm, we optimize the two variables $m_{1,1}$ and $\mathbf{M}_{2,1}$ in (\ref{eq:constrained_final}) alternately: holding one variable fixed while optimizing the other, and vice versa, until convergence. 
We describe the algorithms to optimize the two variables $m_{1,1}$ and $\mathbf{M}_{2,1}$ in order next. 


\subsubsection{Optimizing $m_{1,1}$}
\label{subsec:solve_m11}
When we fix $\mathbf{M}_{2,1}$ and optimize $m_{1,1}$, the objective in (\ref{eq:constrained_final}) is convex and the constraints become linear. We first calculate the gradient of the objective $F$ in (\ref{eq:constrained_final}) with respect to $m_{1,1}$  as
\begin{align}
    \bigtriangledown F(m_{1,1}) = &-\sum_{\{i,j\}}\mathbf{g}_{ij}(1)^2
\exp\{- (\mathbf{g}_{ij}(1)^2 m_{1,1} \nonumber \\
&+ 2 \mathbf{g}_{ij}(1) \mathbf{M}_{2,1}^{\top} \mathbf{g}_{ij}(2))\}\tilde{d}_{i,j},
\end{align}
%\red{why r u not lumping the exponential term involving $\mathbf{M}_{2,2}$ to $d_{i,j}$? why are you not writing out the derivative?} \blue{edited.} 
which is always non-positive. Hence, the minimum objective will be achieved at the upper bound of $m_{1,1}$ in the constraints of (\ref{eq:constrained_final}). The optimal $m_{1,1}$ is thus the upper bound, i.e., $C-\text{tr}(\mathbf{M}_{2,2})$.    
\red{u r just choosing one end as the optimal $m_{1,1}$?} \blue{Modified now. }
% \begin{equation}
%     \bigtriangledown F(m_{1,1}) =-\sum_{\{i,j\}}\mathbf{g}_{ij}(1)^2\exp\{-\mathbf{g}_{ij}(1)^2 m_{1,1} \}d_{i,j},
% \end{equation}
% which is deployed to acquire the solution of gradient descent in each iteration. We then perform proximal mapping of the solution onto the feasible space of constraints, which is linear:
% \begin{equation}
%     \Pi_{T_1}(m_{1,1}) = \{\frac{1}{\theta_{\text{min}}} \mathbf{M}_{2,1}^{\top} \mathbf{M}_{2,1} \leq m_{1,1} \leq C - \text{tr}(\mathbf{M}_{2,2})\}
% \end{equation}
% Each iteration in the PG algorithm can thus be written as
% \begin{equation}
%      m_{1,1}^{l+1} := \Pi_{T_1}(m_{1,1}^l - t \bigtriangledown F(m_{1,1}^l)),
% \end{equation}
% where $t$ is the step size.

\subsubsection{Optimizing $\mathbf{M}_{2,1}$}

When we fix $m_{1,1}$ and optimize $\mathbf{M}_{2,1}$, the objective is convex while the lone constraint for $\mathbf{M}_{2,1}$ forms a convex set. 
In particular, the first constraint in (\ref{eq:constrained_final}) reduces to 
\begin{equation}
    \mathcal{S}=\{\| \mathbf{M}_{2,1} \|_2^2 < \theta_{\text{min}} m_{1,1}\},
\end{equation}
which is a $(K-1)$-dimensional norm ball with radius $\sqrt{\theta_{\text{min}} m_{1,1}}$. 
We now define an indicator function $I_{\mathcal{S}}(\mathbf{M}_{2,1})$:
\begin{equation}
   I_{\mathcal{S}}(\mathbf{M}_{2,1})=
    \left\{
        \begin{array}{lr} 
            0, & \mathbf{M}_{2,1} \in \mathcal{S}  \\
            \infty, & \text{otherwise}
        \end{array}
    \right. 
\end{equation}
We can rewrite the optimization sub-problem for $\mathbf{M}_{2,1}$ as an unconstrained problem by exchanging the convex set constraint with an indicator function in the objective:
\begin{align}
\min_{\mathbf{M}_{2,1}}
    \sum_{\{i,j\}} 
    & \exp\{- (\mathbf{g}_{ij}(1)^2 m_{1,1} + 2 \mathbf{g}_{ij}(1) \mathbf{M}_{2,1}^{\top} \mathbf{g}_{ij}(2))\}\tilde{d}_{i,j} \nonumber \\
    & + I_{\mathcal{S}}(\mathbf{M}_{2,1}).
    \label{eq:solve_M21}
\end{align}  
The first term is convex with respect to $\mathbf{M}_{2,1}$ and differentiable, while the second term $I_{\mathcal{S}}(\mathbf{M}_{2,1})$ is convex but non-differentiable. Hence, we employ \textit{proximal gradient} (PG) \cite{Parikh31} to solve (\ref{eq:solve_M21}).   

Specifically, we first compute the gradient of the first term $F$ in the objective with respect to $\mathbf{M}_{2,1}$ as 
\begin{align}
    \bigtriangledown F(\mathbf{M}_{2,1}) =
    &-2 \sum_{\{i,j\}} \mathbf{g}_{ij}(1) \mathbf{g}_{ij}(2)\exp\{- (\mathbf{g}_{ij}(1)^2 m_{1,1} \nonumber \\
    &  + 2 \mathbf{g}_{ij}(1) \mathbf{M}_{2,1}^{\top} \mathbf{g}_{ij}(2))\}\tilde{d}_{i,j},
\end{align}
which will be adopted in the step of gradient descent. If $ \mathbf{M}_{2,1} \notin \mathcal{S}$ after gradient descent, we perform a proximal mapping $\Pi_{I_{\mathcal{S}}}(\mathbf{v})$ for $\mathbf{v} \in \mathbb{R}^{(K-1) \times 1} $, which is a projection onto the norm ball with radius $\sqrt{\theta_{\text{min}} m_{1,1}}$:
\red{this does not look nice. u need ``if" in the first line. u can simply the notation a bit, because we are talking about a general proximal mapping function, and it can operate on any vector $\mathbf{v}$.} \blue{Modified.}
\begin{equation}
     \Pi_{I_{\mathcal{S}}}(\mathbf{v}) =
    \left\{
        \begin{array}{lr} 
            \mathbf{v}, & \| \mathbf{v} \|_2 \leq \sqrt{\theta_{\text{min}} m_{1,1}}  \\
            \frac{\mathbf{v}}{\| \mathbf{v} \|_2} \cdot \sqrt{\theta_{\text{min}} m_{1,1}}, & \text{otherwise}
        \end{array}
    \right. 
\end{equation}
Then each iteration in the PG algorithm can be written as
\begin{equation}
     \mathbf{M}_{2,1}^{l+1} := \Pi_{I_{\mathcal{S}}}(\mathbf{M}_{2,1}^l - t \bigtriangledown F(\mathbf{M}_{2,1}^l)),
\end{equation}
%\red{the notation is not consistent. Is it $\Pi_{I_{\mathcal{S}}}$? or $\Pi_{\mathcal{S}}$?} \blue{fixed.}
where $t$ is the step size. As discussed in \cite{Parikh31,combettes11}, the algorithm will converge with rate $O(1/l)$ for a fixed step size $t^l = t \in (0,2/L]$, where $L$ is a Lipschitz constant that requires computation of the Hessian of $F$. 
In our experiment, we choose a small step size $t$ empirically, which is small enough to satisfy the Lipschitz smoothness of the objective function.
%\red{u don't know the Lipschitz constant, right? can you bound it? if not, how can u claim your chosen step size $t$ is small enough??} \blue{Not sure if we can bound the Lipschitz constant yet. A backtracking stepsize rule was proposed in case of unknown Lipschitz constant. }

Further, we may reduce the complexity of the proposed algorithm via \textit{accelerated proximal gradient} (APG) \cite{beck09siam,beck09tip,li15apg}. APG is able to accelerate the convergence, by first extrapolating a point from the current point and the previous point and then performaing a proximal gradient step. 
We leave this as our future work.  




% where $\mathbf{c}=[c_1,...,c_m]^T$, and $\mathbf{c}^T\mathbf{M}\mathbf{c}$ is its
% Mahalanobis distance with a matrix $M$. The domain of $M$ is the cone of positive
% semi-definite matrices. Both the objective and constraint in (\ref{eq:optimize_c_constraint}) are convex, and thus can be solved optimally and efficiently.  

% We deploy proximal gradient descent to solve (\ref{eq:optimize_c_constraint}). Firstly, we compute the gradient of the objective $g(\mathbf{M})$:
% \begin{equation}
%     \bigtriangledown g(\mathbf{M}) = -\sum_{\{i,j\}} \exp\{-(\mathbf{f}_i-\mathbf{f}_j)^T \mathbf{M} (\mathbf{f}_i-\mathbf{f}_j) \}d_{i,j} \cdot (\mathbf{f}_i-\mathbf{f}_j)(\mathbf{f}_i-\mathbf{f}_j)^T
% \end{equation}

% According to the constraint in (\ref{eq:optimize_c_constraint}), we project onto the convex spectral set:
% \begin{equation}
%     T = \{\mathbf{M} \succeq 0 ~|~ \text{tr}(\mathbf{M}) \leq C\}
% \end{equation}
% The proximal projection onto $T$ is given by
% \begin{equation}
% \begin{split}
% \Pi_T(\mathbf{M}) &=\mathbf{U} \textbf{diag}(\Pi_S(\sigma(\mathbf{M}))) \mathbf{U}^T \\ &=\sum_{i=1}^K \text{min}\{\text{max}\{\lambda_i,0\},C\}\mathbf{u}_i\mathbf{u}_i^T,
% \end{split}
% \end{equation}
% where $\mathbf{U}$ is the matrix of eigenvectors $\mathbf{u}_i$ of $\mathbf{M}$ and $\sigma(\mathbf{M})$ is the diagonal matrix of eigenvalues $\lambda_i$ of $\mathbf{M}$. The operation of $\text{max}\{\lambda_i,0\}$ ensures $\mathbf{M}$ is positive semi-definite, while $\text{min}\{\cdot,C\}$ is necessary for the constraint $\text{tr}(\mathbf{M}) \leq C$.

% We then have the PG iteration:
% \begin{equation}
%     \mathbf{M}^{l+1} := \Pi_T(\mathbf{M}^l - t \bigtriangledown g(\mathbf{M}^l)).
% \end{equation}

   
% \begin{equation}
% \begin{split}
% &\min_{c_1,c_2}
%     \sum_{\{i,j\}}\exp{\left(-c_1\|\vec{p}_s-\vec{p}_t\|_2^2-c_2\left| \sin \left \langle \mathbf{n}_s, \mathbf{n}_t \right \rangle \right| \right)}\|\mathbf{p}_i-\mathbf{p}_j\|_2^2+\beta\|\mathbf{c}\|_2^2,\\
% & \quad \text{s.t.} \quad \, c_1 > 0, c_2 > 0.
% \label{eq:optimize_c_constraint}
% \end{split}
% \end{equation}
 

%a function of the angle between the normals of neighboring points into the weight function.  



%In (\ref{eq:graph_weight}), the exponential term describes the relative distance between $\mathbf{p}_i$ and $\mathbf{p}_j$, as widely adopted in the literature. Further, the cosine term captures the similarity between the direction of normals at $\mathbf{p}_i$ and $\mathbf{p}_j$. If the normal angle is large and even reaches $\pi/2$, then the cosine term tends to $0$, resulting in a small weight even when the relative distance between $\mathbf{p}_i$ and $\mathbf{p}_j$ is small. Hence, this term penalizes corresponding points with large difference in the normal direction, i.e., when the two points reside on local surfaces with different orientations. We apply the PCA-based method \cite{hoppe92} to estimate surface normals from point clouds based on local neighborhoods of each point, which is robust to noise.  
%
%In particular, $\sigma$ decides the radius of the neighborhood and the distribution of edge weights, which has substantial impact on the denoising performance. 

%\begin{equation}
%\min_{\sigma}
%    \sum_{\{i,j\}}\sum_{c \in \{x,y,z\}}\exp{\left(-\frac{\|\mathbf{p}_i-\mathbf{p}_j\|^2}{ \sigma ^2}\right)} \cdot \left| \cos \left \langle \mathbf{n}_s, \mathbf{n}_t \right \rangle \right|(p_s^c-p_t^c)^2.
%    \label{eq:optimize_L}
%\end{equation}







% \subsection{Computational Complexity Analysis}

% The computational complexity of our algorithm can be deduced as follows:
% \begin{itemize}
%     \item We use KD-tree for the $k$-nearest-neighbor searches. The cost of the $k$-nearest-neighbor search for all points is $\mathcal{O}(kN \log N)$.
%     \item We need to run the RPCA solver to estimate the normal on each point using its $k$-nearest-neighbor. The cost of the RPCA solver on each point is $\mathcal{O}(tk)$ \cite{mattei}, where $t$ is the number of iterations. For all points, the cost is $\mathcal{O}(tkN)$.
%     \item Constructing $M$ patches still requires $k$-NN search, and the cost is $\mathcal{O}(kM \log N)$.
%     \item For graph construction, the $\varepsilon$-nearest-patch to be connected can be found in $\mathcal{O}(\varepsilon M \log M)$ time.
%     \item For the weight computation, the cost is $\mathcal{O}(\varepsilon k^2 M)$.
%     \item The cost of CG-based algorithm to solve the optimization problem is $\mathcal{O}(m \sqrt{\kappa})$ \cite{shewchuk1994introduction}, where $m$ is the number of non-zero entries in the matrix, and $\kappa$ is the condition number of the matrix. In our problem, the Laplacian matrix is sparse, and thus $m \ll N^2$.

% Overall, the running time of our algorithm depends on four parameters (1) the number of nearest neighbors, (2) the number of iterations to run the RPCA normal estimation, (3) the number of patches, and (4) the number of nearest patch neighbors.
